Hierarchy Denoising Recursive Autoencoders for 3D Scene Layout Prediction

Indoor scenes exhibit rich hierarchical structure in 3D object layouts. Many tasks in 3D scene understanding can benefit from reasoning jointly about the hierarchical context of a scene, and the identities of objects. We present a variational denoising recursive autoencoder (VDRAE) that generates and iteratively refines a hierarchical representation of 3D object layouts, interleaving bottom-up encoding for context aggregation and top-down decoding for propagation. We train our VDRAE on large-scale 3D scene datasets to predict both instance-level segmentations and a 3D object detections from an over-segmentation of an input point cloud. We show that our VDRAE improves object detection performance on real-world 3D point cloud datasets compared to baselines from prior work.

==> figures/conver_plot.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure}[t!] \centering
	\begin{overpic}[width=1.0\linewidth,tics=10]{figures/images/conver_plot}%,grid
	\end{overpic}
    \caption{
    Average number of 3D object nodes in the predicted hierarchy plotted against iteration count during refinement of the 3D scene layout in Matterport3D test set scenes.
    We see that the total number of nodes converges, confirming our empirical observation that our hierarchy refinement algorithm converges within about 5 iterations for the datasets we tested.
    }
    \label{fig:conver_plot}
    %\vspace{-6pt}
\end{figure} 

==> figures/decoder.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure}
\includegraphics[width=1.0\linewidth]{figures/images/decoder}
\caption{
Our decoder architecture takes an aggregated feature and decodes it to pairs of node features (here shown as $x_l^{dec}$ and $x_r^{dec}$.
From these features, we predict several targets: whether the node corresponds to a 3D object detection or not ($o_n$), the category of the object detection $c_n$ and the parameters of the bounding box for the detection $t_n$.
}
%\vspace{-2em}
\label{fig:decoder}
\end{figure}

==> figures/encoder.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure}
\includegraphics[width=1.0\linewidth]{figures/images/encoder}
\caption{
Our encoder architecture takes a point cloud segment as input for each node and then combines PointCNN features, oriented bounding box (OBB) parameters for the node, and a feature encoding that from node's child nodes.
These features are passed through $\text{FC}$ layers to produce the encoding $x_i^{enc}$ of the specific node, and then individual node encoding pairs are combined through $f_{enc}$ to produce the encoding feature $x_p^{enc}$ for their parent node.
}
%\vspace{-2em}
\label{fig:encoder}
\end{figure}

==> figures/recur_loss.tex <==
%!TEX root = ../sceneparse.tex

\begin{figure}[t!] \centering
	\begin{overpic}[width=1.0\linewidth,tics=10]{figures/images/recursive_loss}%,grid
    \put(23,-3){\small (a)}
    \put(75,-3){\small (b)}
	\end{overpic}
    \caption{
    To train our denoising RAE network, we define a \emph{recursive tree-to-tree loss}.
    We first match source and target hierarchy subtrees through recursive node assignment \textbf{(a)}.
    This matching enables backpropagation of the recursive loss through the tree structure of the hierarchy \textbf{(b)}.
    }
    \label{fig:recurloss}
    \vspace{-6pt}
\end{figure} 

==> sections/convergence.tex <==
\section{Discussion of Convergence of 3D Scene Layout Refinement}
\label{sec:convergence}

\input{sections/algo_rae.tex}

Algorithm 1 of the main paper (reproduced here for convenience), presents an approach for iteratively applying our VDRAE to improve 3D scene layout prediction.
Here we discuss the converge properties of our algorithm.

The algorithm iterates until the structure of the hierarchy between iterations remains unchanged.
During each iteration, the resulting hierarchy is determined by the scaled affinity $E(u,v) = e_c e_a$ where $$
e_c(u,v) = \left\{\begin{array}{rr}
  -\text{log}(1-c_s), & u \text{ and } v \text{ in same leaf node $s$} \\
  0.1, & \text{otherwise}
\end{array}\right.
$$
and $c_s$ is the classification confidence of node $s$ to be labeled as `object'.
Note that this changes only when $c_s$ changes.
For more confident groupings of $u$ and $v$, $c_s$ approaches $1$, so $e_c$ approaches $+\infty$, making it more expensive to separate $u,v$.
In contrast, for less confident groupings, both $c_s$ and $e_c$ is close to zero, resulting in a weaker bond between the two nodes.

When we iterate, we will naturally keep the grouping of subtrees $u,v$ whose parent node $s$ has a high classification confidence $c_s$, and adjust the grouping of the nodes that has a less confident $c_s$.
Thus, at each iteration, we only need to consider what happens to nodes with low $c_s$ (we can consider nodes with high $c_s$ to be fixed).

After each iteration, we will have alternate groupings that result in either 1)  more nodes with a higher $c_s$ or 2) no more nodes with high $c_s$.  In case 2), because the nodes have low $c_s$, they are not object nodes and so do not affect the overall object detection result.  Thus the structure of the hierarchy does not change between iterations and the algorithm is converged in this scenario.  In case 1), there are increasing number of nodes with high $c_s$ values corresponding to more object nodes and we will continue to iterate.  However, every time, since we have a finite number of nodes, the number of nodes going from low $c_s$ to high $c_s$ will decrease until there are no low $c_s$ nodes left.  In this case, all nodes will belong to some single object node, and the hierarchy structure will have converged as well.

This is a high-level discussion of the convergence behavior of our layout refinement approach.
In practice, we observe that 3D scene layouts converge to non-changing hierarchy structure within $5$ iterations.
This is confirmed also by the plot in \Cref{fig:conver_plot} which shows the average number of detected hierarchy object nodes against iteration count across test scenes from the Matterport3D test set.
We leave a more thorough and formal discussion of the convergence properties of VDRAE-based 3D scene layout refinement to future work.

% Main idea: keep the grouping order of subtrees whose root node has a high confidence to be classified as a single object; adjust the grouping order of the rest nodes


%How it works
%In the next iteration, the rest nodes, which not belong to any high confidence subtrees, will find a new grouping order. This task is easier than to build a tree from scratch, because subtrees with high confidence are fixed.

%Why it will converge

%There will be two consequence after each iteration: 1) we don’t have more nodes with high confidence appear, so the hierarchy keep unchanged; 2) we have more nodes with high confidence so we keep adjusting the hierarchy;

%If the algorithm goes to 1) some time, it is converged because the hierarchy and object detection result will not be changed any more

%If the algorithm goes to 2) all the time, the final status will be: all the nodes belong to some single objects, so It converges too.

==> sections/instance_segmentation.tex <==
%!TEX root = sceneparse.tex

\section{3D Instance Segmentation Evaluation}
\label{sec:inst_seg}

In \Cref{tab:inst_seg_s3dis} and \Cref{tab:inst_seg_mp}, we report results on the 3D instance segementation task.
Though the goal of our method is not to do 3D instance segmentation, such segmentations are produced implicitly when segments from the point cloud are assigned to detected 3D object nodes in our layout hierarchy, each with a specific category label.
We see that our approach outperforms the baseline from the state-of-the-art 3D instance semantic segmentation approach~\cite{wang2018sgpn}.

\begin{table*}
\footnotesize\centering
\begin{tabular}{lccccccc}
\toprule
& Column & Chair & Table & Bookcase & Sofa & Board & mAP \\
\midrule
%Seg-Cluster~\cite{wang2018sgpn} & 0.159 & 0.103 & 0.226 & 0.433 & 0.039 & 0.107 & 0.178 \\
SGPN~\cite{wang2018sgpn} & 0.607 & 0.408 & 0.469 & 0.476 & 0.064 & 0.111 & 0.356 \\
\midrule
Ours & \textbf{0.623} & \textbf{0.462} & \textbf{0.537} & 0.449 & \textbf{0.451} & \textbf{0.415} & \textbf{0.445} \\
\bottomrule
\end{tabular}
\caption{
Comparison of our approach against prior work on instance segmentation on the S3DIS dataset.
Values report average precision with IoU threshold 0.5.
%\todo{Add Matterport3D numbers (can remove SegCluster), will make it easier for us to argue why we don't do architecture categories in S3DIS.}
}
\label{tab:inst_seg_s3dis}
\end{table*}


\begin{table*}
\footnotesize\centering
\begin{tabular}{lcccccccccccc}
\toprule
& Chair & Table & Cabinet & Cushion & Sofa & Bed & Sink & Toilet & TV & Bathtub & Lighting & mAP \\
\midrule
SGPN~\cite{wang2018sgpn} & 0.241 & 0.176 & 0.036 & 0.159 & 0.267 & 0.304 & 0.110 & 0.149 & 0.042 & 0.063 & 0.057 & 0.146\\
\midrule
Ours & \textbf{0.305} & \textbf{0.210} & \textbf{0.062} & \textbf{0.217} & 0.248 & \textbf{0.350} & \textbf{0.136} & \textbf{0.329} & \textbf{0.057} & \textbf{0.121} & \textbf{0.106} & \textbf{0.195} \\
\bottomrule
\end{tabular}
\caption{
Comparison of our approach against prior work on instance segmentation on the Matterport3D dataset.
Values report average precision with IoU threshold 0.5.
}
\label{tab:inst_seg_mp}
\end{table*}

==> sections/more_results.tex <==
%!TEX root = sceneparse.tex

\section{Qualitative Comparison of 3D Scene Layout Prediction Results}
\label{sec:compare}

\Cref{fig:compare} shows additional qualitative comparisons of our VDRAE 3D layout prediction to ground truth and results using SGPN~\cite{wang2018sgpn} on Matterport3D test scenes.
In general, we see that our VDRAE approach matches the ground truth layouts more closely than the baseline approach.
%Particular examples where addition or merging of detected object boxes was necessary include the lamps on the nightstands in the top left, the sink in the second row on the left, and the fridge in the last row on the left.
These results demonstrate that our hierarchical encoding of the 3D layout and iterative refinement through the trained VDRAE can lead to improvements in 3D object detection.


==> sections/overview.tex <==
%!TEX root = ../sceneparse.tex

\section{Overview}
\label{sec:overview}

The input to our method is a 3D point cloud representing an indoor scene, possibly with noise and incompleteness.
The output is a set of objects represented by oriented bounding boxes (OBBs), each with a category label.
We will use $\mathcal{B}$ to refer to this set of bounding boxes with labels.
%These OBBs can be replaced by CAD models retrieved from a shape database.
Starting from an initial over-segmentation of candidate parts for object detections (\Cref{sec:overseg}), our method jointly optimizes the configuration of multiple objects, through a hierarchical context aggregation and propagation.
Starting from an initial over-segmentation, we construct a hierarchy $h$ used for context propagation (\Cref{sec:hierarchy}).
Having built the hierarchy, we iteratively refine the object detection and the hierarchy based on a recursive autoencoder network (\Cref{sec:recursive}).
We call the combination of the object detections and the constructed hierarchy $\{\mathcal{B},h\}$ the object layout of the scene.
Our output set of labeled bounding boxes $\mathcal{B}$ contains a category label for all object detections, or a label indicating a particular box is not an object. \todo{check}
Figure~\ref{fig:overview} shows an overview of our method.

\paragraph{Initial over-segmentation.}
Our approach creates an initial set of segment OBBs from the input using an over-segmentation, which we then merge into object detections, and recursively refine and classify.
We demonstrate that we can reliably detect objects from this initial input by leveraging a hierarchical encoding of the 3D object layout.

\paragraph{Hierarchy construction.}
Given a set of objects, we build the hierarchy $h$ using object segment pair affinities and a normalized cuts approach.
The inter-segment affinities are learned through supervised binary classification of co-occurring object segments and objects based on segment geometric and appearance features in the training scenes.
Given a test scene we predict affinities for the initial over-segmentation and perform a recursive binary segmentation over the graph utilizing normalized cuts to construct a hierarchy~\cite{shi2000normalized}.

\paragraph{Training and testing the recursive autoencoder.}
We then employ a recursive autoencoder (RAE) for context aggregation and propagation.
To refine the layout of object detections, we train a variational denoising RAE (a probabilistic generative model, abbreviated as VDRAE) which captures the manifold of plausible scene layouts.
Passing an imperfect scene layout through this trained VDRAE ``snaps'' the layout onto the learned manifold by refining, adding or removing object nodes.
To deal with highly inaccurate initial object detections, we use an iterative layout optimization in which each iteration interleaves VDRAE testing and hierarchy rebuilding.
This process is repeated until convergence defined as the detected object bounding boxes becoming stable.

